Pressure profiles and mass estimates using high-resolution Sunyaev-Zel'dovich effect observations of Zwicky 3146 with MUSTANG-2

The galaxy cluster Zwicky 3146 is a sloshing cool core cluster at $z=0.291$ that in X-ray imaging does not appear to exhibit significant pressure substructure in the intracluster medium (ICM). The published $M_{500}$ values range between $3.88^{+0.62}_{-0.58}$ to $22.50 \pm 7.58 \times 10^{14}$ M$_{\odot}$, where ICM-based estimates with reported errors $<20$\% suggest that we should expect to find a mass between $6.53^{+0.44}_{-0.44} \times 10^{14}$ M$_{\odot}$ (from Planck, with an $8.4\sigma$ detection) and $8.52^{+1.77}_{-1.47} \times 10^{14}$ M$_{\odot}$ (from ACT, with a $14\sigma$ detection). This broad range of masses is suggestive that there is ample room for improvement for all methods. Here, we investigate the ability to estimate the mass of Zwicky 3146 via the Sunyaev-Zel'dovich (SZ) effect with data taken at 90 GHz by MUSTANG-2 to a noise level better than $15\ \mu$K at the center, and a cluster detection of $104\sigma$. We derive a pressure profile from our SZ data which is in excellent agreement with that derived from X-ray data. From our SZ-derived pressure profiles, we infer $M_{500}$ and $M_{2500}$ via three methods -- $Y$-$M$ scaling relations, the virial theorem, and hydrostatic equilibrium -- where we employ X-ray constraints from \emph{XMM-Newton} on the electron density profile when assuming hydrostatic equilibrium. Depending on the model and estimation method, our $M_{500}$ estimates range from $6.23 \pm 0.59$ to $10.6 \pm 0.95 \times 10^{14}$ M$_{\odot}$, where our estimate from hydrostatic equilibrium, is $8.29^{+1.93}_{-1.24}$ ($\pm 19.1$\% stat) ${}^{+0.74}_{-0.68}$ ($\pm 8.6$\% sys, calibration) $\times 10^{14}$ M$_{\odot}$. Our fiducial mass, derived from a $Y$-$M$ relation is $8.16^{+0.44}_{-0.54}$ ($\pm 5.5$\% stat) ${}^{+0.46}_{-0.43}$ ($\pm 5.5$\% sys, $Y$-$M$) ${}^{+0.59}_{-0.55}$ ($\pm 7.0$\% sys, cal.) $\times 10^{14}$ M$_{\odot}$.

==> CommentConsolidation.tex <==
\subsection{Suggestions}

\begin{enumerate}
    \item Move sections to appendices; clean up the draft
    
\end{enumerate}

%\author{
%  Order TBD ,
%  Charles E. Romero\altaffilmark{1},
%  Jonathan Sievers\altaffilmark{2},
%  Vittorio Ghirardini\altaffilmark{3},
%  Simon Dicker\altaffilmark{1},
%  Simona Giaccintucci\altaffilmark{4},
%  Tony Mroczkowski\altaffilmark{5},
%  Massimo Gaspari\altaffilmark{6}
%  Brian S.\ Mason\altaffilmark{3},
%  Craig Sarazin\altaffilmark{7},
%  Mark Devlin\altaffilmark{1},
%  Sara Stanchfield\altaffilmark{1}
%}		
%\date{\today}
%
%\altaffiltext{1}{Department of Physics and Astronomy, University of
%  Pennsylvania, 209 South 33rd Street, Philadelphia, PA, 19104, USA}
%\altaffiltext{2}{Department of Physics, McGill University, 3600 University Street
%%Montreal, QC H3A 2T8, Canada}  
%\altaffiltext{3}{National Radio Astronomy Observatory, 520 Edgemont
%  Rd., Charlottesville VA 22903, USA} 
%\altaffiltext{4}{U.S. Naval Research Laboratory, 4555 Overlook Avenue SW, Washington, DC 20375, USA}
%\altaffiltext{5}{ESO - European Southern Observatory, Karl-Schwarzschild-Str.\ 2, D-85748 Garching b.\ M\"unchen, %Germany}
%\altaffiltext{5}{Department of Astrophysical Sciences, Princeton University, 4 Ivy Lane,
%Princeton, NJ 08544}
%\altaffiltext{6}{Department of Astronomy, University of Virginia,
%  P.O. Box 400325, Charlottesville, VA 22901, USA}


==> ProseZwMasses.tex <==
% Nothing to see here


==> Residuals.tex <==
\begin{deluxetable}{l | c c c c c c}
\tabletypesize{\scriptsize}
\tablecolumns{7}
\tablewidth{0pt}
\tablecaption{Residual Gaussian Parameters \label{tbl:resid_pars}}
\tablehead{ & \colhead{$A$} & \colhead{RA$_{0}$} & \colhead{$\delta_{0}$} & \colhead{FWHM$_{a}$} & \colhead{FWHM$_{b}$} & $R_p$ \\
 & \colhead{($\mu$K} & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(\arcsec)} & \colhead{(\arcsec)} & \colhead{(\arcsec)} }
\startdata
    Minkasi, SW & 73.4  & 10:23:38.35 & 04:10:57.45 & 31.3  & 18.7  & 23.7 \\
    Minkasi, NE & 33.6  & 10:23:40.79 & 04:11:32.64 & 31.3  & 18.7  & 27.9 \\
    MIDAS, SW     & 42.8  & 10:23:38.69 & 04:11:0.17  & 12.9  & 11.1  & 17.9 \\
    MIDAS, NE     & 43.7  & 10:23:41.49 & 04:11:28.26 & 12.9  & 11.1  & 32.5 \\
\enddata
\tablecomments{ Fitted two dimensional Gaussian parameters. The shape and orientation of the Gaussian between the SW and NE residuals are linked, while the centroids and amplitudes are allowed to vary individually. The final column, $R_p$, gives the radial separation from the central point source (yellow cross in Figure~\ref{fig:zw3146_residuals}). }
\end{deluxetable}


==> excess_packages.tex <==
%\documentclass[iop,numberedappendix,apj]{emulateapj}
%\documentclass{emulateapj}
%\documentclass{article}
%\documentclass[iop,onecolumn,apj]{emulateapj}
%\documentclass[iop,numberedappendix,apj]{aastex}
%\usepackage{color}
%\usepackage{amssymb}
%\usepackage{natbib}
%\usepackage{graphicx}
%\usepackage{url}
%\usepackage[utf8]{inputenc}
%\usepackage{deluxetable} % Included in emulate apj
%\usepackage[table,x11names]{xcolor}


==> latex_commands.tex <==
\newcommand {\apgt} {\ {\raise-.5ex\hbox{$\buildrel>\over\sim$}}\ }
\newcommand {\aplt} {\ {\raise-.5ex\hbox{$\buildrel<\over\sim$}}\ }
\newcommand{\dmod}{\overrightarrow{d}_{mod}}
\newcommand{\dvec}{\overrightarrow{d}}
\newcommand{\avec}{\overrightarrow{a}}
\newcommand{\asec}{$^{\prime \prime}$}
\newcommand{\asecs}{$^{\prime \prime}\ $}
\newcommand{\amin}{$^{\prime}$}
\newcommand{\amins}{$^{\prime}\ $}
\newcommand{\sigT}{\mbox{$\sigma_{\mbox{\tiny T}}$}}
\newcommand{\Tcmb}{\mbox{$T_{\mbox{\tiny CMB}}$}}
\newcommand{\kB}{\mbox{$k_{\mbox{\tiny B}}$}}
\newcommand{\kBT}{\mbox{$k_{\mbox{\tiny B}}T_{\mbox{\tiny e}}$}}
\newcommand{\nH}{\mbox{$n_{\mbox{\tiny H}}$}}
\newcommand{\NH}{\mbox{$N_{\mbox{\tiny H}}$}}
\newcommand{\LameH}{\mbox{$\Lambda_{e \mbox{\tiny H}}$}}
\newcommand{\Lamee}{\mbox{$\Lambda_{ee}$}}
\newcommand{\rhogas}{\mbox{$\rho_{\mbox{\scriptsize gas}}$}}
\newcommand{\rhotot}{\mbox{$\rho_{\mbox{\scriptsize tot}}$}}
\newcommand{\Mgas}{\mbox{$M_{\mbox{\scriptsize gas}}$}}
\newcommand{\Mtot}{\mbox{$M_{\mbox{\scriptsize tot}}$}}
\newcommand{\Mvir}{\mbox{$M_{\mbox{\scriptsize vir}}$}}
\newcommand{\Yint}{\mbox{$Y_{\mbox{\scriptsize int}}$}}
\newcommand{\Ycyl}{\mbox{$Y_{\mbox{\scriptsize cyl}}$}}
\newcommand{\Ysph}{\mbox{$Y_{\mbox{\scriptsize sph}}$}}
\newcommand{\fgas}{\mbox{$f_{\mbox{\scriptsize gas}}$}}
\newcommand{\LCDM}{\mbox{$\Lambda$CDM}}
\newcommand{\Pe}{\mbox{$P_{\mbox{\scriptsize e}}$}}
\newcommand{\msun}{$M_{\odot}$}
\newcommand{\etal}{{\it et al.}}
\newcommand{\mJy}{\,{\rm mJy} }
\newcommand{\um}{\,\mu {\rm m} }
\newcommand{\mJySr}{\,{\rm MJy/Sr} }
\newcommand{\mJyBm}{\,{\rm mJy/Bm} }
\newcommand{\mK}{\,{\rm mK} }
\newcommand{\K}{\,{\rm K} }
\newcommand{\uJy}{\,{\rm \mu Jy} }
\newcommand{\uK}{\,{\rm \mu K} }
\newcommand{\kHz}{\, {\rm kHz} }
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}
\newcommand{\aips}{{\tt AIPS++}}
\newcommand{\nusp}{\nu_{sp}}
\newcommand{\ghz}{{\, \rm GHz}}
\newcommand{\db}{{\, \rm dB}}
\newcommand{\degsqr}{\, {\rm deg^2}}
\newcommand{\Tew}{\mbox{$T_{\mathrm{ew}}$}}
\newcommand{\Tspec}{\mbox{$T_{\mathrm{spec}}$}}
\newcommand{\chandra}{{\it Chandra}}
\newcommand{\asca}{{ASCA}}
\newcommand{\wmap}{{WMAP}}
\newcommand{\rosat}{{ROSAT}}
\newcommand{\xmm}{{XMM-{\it Newton}}}
\newcommand{\planck}{{\it Planck}}
\newcommand{\hubble}{{\it Hubble}}
\newcommand{\rxj}{RX J1347.5-1145}
\newcommand{\clj}{CL J1226.9+3332}
\newcommand{\macsa}{MACS J0647.7+7015}
\newcommand{\macsb}{MACS J1206.2-0847}
\newcommand{\macsc}{MACS J0717.5+3745}
\newcommand{\macsd}{MACS J1423.8+2404}
\newcommand{\macse}{MACS J0329.6-0211}
\newcommand{\macsf}{MACS J0429-0253}
\newcommand{\macsg}{MACS J0744.9+3927}
\newcommand{\macsh}{MACS J1149+2223}
\newcommand{\macsi}{MACS J1115+0130}
\newcommand{\Tx}{\mbox{$T_{\mbox{\tiny X}}$}}
\newcommand{\te}{\mbox{$T_{\mbox{\tiny e}}$}}
\newcommand{\mec}{\mbox{$m_{\mbox{\tiny e}} c^2$}}
\newcommand{\dene}{\mbox{$n_{\mbox{\tiny e}}$}}
\newcommand{\denesq}{\mbox{$n^2_{\mbox{\tiny e}}$}}
\newcommand{\yx}{\mbox{$Y_{\mbox{\tiny X}}$}}
\newcommand{\ysze}{\mbox{$Y_{\mbox{\tiny tSZE}}$}}
\newcommand{\sx}{\mbox{$S_{\mbox{\tiny X}}$}}
\newcommand{\Itsz}{\mbox{$I_{\mbox{\tiny tSZE}}$}}
\newcommand{\Iksz}{\mbox{$I_{\mbox{\tiny kSZE}}$}}
\newcommand{\chisq}{\mbox{$\chi^{2}$}}
\newcommand{\chired}{\mbox{$\chi^{2}_{red}$}}
\newcommand{\jcap}{{JCAP}}

==> macros.tex <==

%--- VARIOUS
\newcommand{\ojo}{\fbox{\bf !`$\odot$j$\odot$!}} 
%\newcommand{\cita}{\citeasnoun}
%\newcommand{\cites}{\citeaffixed}
\newcommand{\lai}{\'{\i}}
\newcommand{\y}{{\it y\ }}
\newcommand{\titlebar}{\rule{15cm}{1mm}\\[2.pt]\rule{15cm}{0.4mm}\\} 

%--- UNITS
\newcommand{\arcmin}{\hbox{$^\prime$}}               % arcmin
\newcommand{\arcsec}{\hbox{$^{\prime\prime}$}}       % arcsec
\newcommand{\kms}{ km\ s$^{-1}$}                     % km s-1
\newcommand{\ergs}{erg s$^{-1}$}                     % erg s-1
\newcommand{\ergsM}{erg s$^{-1}$Mpc$^{-3}$}          % erg s-1 Mpc-3
\newcommand{\sen}{mJy/$\sqrt{\rm Hz}$}               % Unidades de sensibilidad
\newcommand{\micron}{\rm \mu m}                            % Micras!!!
\newcommand{\cm}{{\rm cm}}
\newcommand{\mm}{{\rm mm}}


\definecolor{DarkGreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{purple}{rgb}{0.5, 0.0, 0.5}
\definecolor{red}{rgb}{1, 0.0, 0.0}
\definecolor{green}{rgb}{0, 1.0, 0.0}

 
%%\newcommand{\dg}{$^\circ$} 
\newcommand{\rHz}{$\rm\mu\mbox{K}\,\mbox{s}^{1/2}$} 
\newcommand{\JyHz}{$\rm mJy\,s^{\frac{1}{2}}$}

%\newcommand{\JyHz}{$\mbox{Jy}\,\mbox{s}^{1/2}$} 
\newcommand{\op}[1]{\mbox{$\tau_{\mbox{\tiny #1~GHz}} $}} 
\newcommand{\HII}{$\mathrm H\:II$} 
\newcommand{\et}{{\it et al. }} 
 

\newcommand{\ergseq}{{\rm erg}\: {\rm s}^{-1}\:}     % erg s-1  (eqn)
\newcommand{\Hub}{km\ s$^{-1}$ Mpc$^{-1}$}           % km s-1 Mpc-1

%Solar:
\newcommand{\Msun}{$M_{\odot}$}                       % M_o 
\newcommand{\Lsun}{$L_{\odot}$}                       % L_o 
\newcommand{\MJ}{$M_J$}                                         % M_Jup
\newcommand{\ME}{$M_{\oplus}$}                          % M_Earth
\newcommand{\Moon}{$M_{Moon}$}                          % M_Moon



%Cosmology:
\newcommand{\Om}{$\Omega_{\rm M}$}
\newcommand{\Ol}{$\Omega_\Lambda$}
\newcommand{\Ok}{$\Omega_k$}


%----------------------- BIBTEX --------------------------
%--- JOURNALS
\newcommand{\apj}{\rm ApJ}
\newcommand{\apjl}{\rm ApJL}
\newcommand{\apjs}{\rm ApJS}
\newcommand{\aaps}{\rm A$\&$AS}
\newcommand{\aap}{\rm A$\&$A}
\newcommand{\aapr}{\rm A$\&$AR}
\newcommand{\mnras}{\rm MNRAS}
%\newcommand{\jcap}{\rm JCAP}
\newcommand{\aj}{\rm Astron. J.}
\newcommand{\araa}{\rm ARAA}
\newcommand{\nat}{\rm Nature}
\newcommand{\pasj}{\rm PASJ}
\newcommand{\ASP}{\rm ASP COnference Series}
\newcommand{\CASP}{\rm Comm. Astrophys. Space Phys.}
\newcommand{\astroph}{\rm astro-ph/}
\newcommand{\apss}{\rm Ap\&SS}%          % Astrophysics and Space Science
\newcommand{\qjras}{\rm QJRAS}%          % Quarterly Journal of the RAS
\newcommand{\pasp}{\rm PASP}%          % Publications of the ASP
\newcommand{\physrep}{\rm Phys. Rep.}
\newcommand{\prd}{\rm Phys/ Rev. D}

\def\aplett{{\it Astrophys.~Lett.}} % Astrophysics Letters
\def\ao{{\it Appl.~Opt.}}           % Applied Optics

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

\def\K{{\rm K}}
\def\milliK{{\rm mK}}
\def\mK{\, {\rm \mu K}}
\def\muK{\, {\rm \mu K}}
\def\muJy{\, {\rm \mu Jy}}
\def\MJy{{\rm MJy}}
\def\Jy{\, {\rm Jy}}
\def\mJy{\, {\rm mJy}}
\def\sr{{\rm sr}}
\def\MJysr{\MJy/\sr}
\def\Mpc{{\rm Mpc}}
\def\GHz{{\rm GHz}}
\def\specint{{I_\nu}}
\def\bfzero{{\bf 0}}

\def\icm{${\rm cm}^{-1}\;$}
\def\3he{$^3{\rm He}$}
\def\arcdeg{\hbox{$^\circ$}}
\def\kusd{{K\$\phantom{0}}} %$
\def\et{{\it et al.}}
\def\COBE{{\sl COBE}}
\def\TBD{{\bf TBD}}

\def\blast{{\sl BLAST}}
\def\blastp{{\sl BLAST-pol}}
\newcommand{\boom}{{\it Boomerang}}
\newcommand{\map}{{\it MAP}}

%\input{aas_macros.sty}
%
% Hyphenations
%
\hyphenation{CMBR}
\hyphenation{bolo-meters}
\hyphenation{an-iso-tropy}


%--- BOOKS
\newcommand{\peacock}{\rm Cambridge University Press }
\newcommand{\avishai}{\rm Cambridge University Press }
\newcommand{\peebles}{\rm Princeton University Press }

%---------------------------------------------------------
\def\lsim{\mathrel{\lower2.5pt\vbox{\lineskip=0pt\baselineskip=0pt
           \hbox{$<$}\hbox{$\sim$}}}}

\def\gsim{\mathrel{\lower2.5pt\vbox{\lineskip=0pt\baselineskip=0pt
           \hbox{$>$}\hbox{$\sim$}}}}





